Can Vision-Language Models Evaluate Handwritten Math?

Recent advancements in Vision-Language Models (VLMs) have opened new possibilities in automatic grading of handwritten student responses, particularly in mathematics. However, a comprehensive study to test the ability of VLMs to evaluate and reason over handwritten content remains absent. To address this gap, we introduce FERMAT, a benchmark designed to assess the ability of VLMs to detect, localize and correct errors in handwritten mathematical content. FERMAT spans four key error dimensions - computational, conceptual, notational, and presentation - and comprises over 2,200 handwritten math solutions derived from 609 manually curated problems from grades 7-12 with intentionally introduced perturbations. Using FERMAT we benchmark nine VLMs across three tasks: error detection, localization, and correction. Our results reveal significant shortcomings in current VLMs in reasoning over handwritten text, with Gemini-1.5-Pro achieving the highest error correction rate (77%). We also observed that some models struggle with processing handwritten content, as their accuracy improves when handwritten inputs are replaced with printed text or images. These findings highlight the limitations of current VLMs and reveal new avenues for improvement. We release FERMAT and all the associated resources in the open-source to drive further research.

==> tables/table2_perturbation_stats.tex <==
\setlength{\tabcolsep}{0pt} % Adjust column spacing
\begin{table}[!t] % Use 't' to place the table at the top of the column
\renewcommand{\arraystretch}{1.1} % Adjust row spacing
\centering
\begin{tabular}{lr}

\toprule
\textbf{Category} & \textbf{\# Instances} \\
\midrule

\rowcolor{computational_bg}
\textbf{Computational (CO)} & \textbf{611} \\
\quad\textsc{Final Number} & 156 \\ 
\quad\textsc{Intermediate Calculation} & 100 \\ 
\quad\textsc{Non-Propagated Step Error} & 80 \\ 
\quad\textsc{Propagated Step Error} & 108 \\
\quad\textsc{Copy Error} & 167 \\
\midrule
\rowcolor{conceptual_bg}
\textbf{Conceptual (CP)} & \textbf{609} \\
\quad\textsc{Theorem Misapplication} & 62 \\ 
\quad\textsc{Misinterpret Question} & 145 \\
\quad\textsc{Invalid Assumption} & 122 \\
\quad\textsc{Outright Incorrect Fact} & 143 \\
\quad\textsc{Formula Misuse} & 137 \\
\midrule
\rowcolor{notational_bg}
\textbf{Notational (NO)} & \textbf{255} \\
\quad\textsc{Symbol Error} & 81 \\ 
\quad\textsc{Operator Swap} & 115 \\ 
\quad\textsc{Misplaced Parentheses} & 59 \\ 
\midrule
\rowcolor{presentation_bg}
\textbf{Presentation (PR)} & \textbf{429} \\
\quad\textsc{Format Ignored} & 47 \\
\quad\textsc{Terminology Swap} & 25 \\
\quad\textsc{Logic Disruption} & 101 \\
\quad\textsc{Contextual Swap} & 43 \\ 
\quad\textsc{Variable Misnaming} & 67 \\
\quad\textsc{Incorrect Units} & 146 \\
\midrule
\rowcolor{superficial_bg}
\textbf{Superficial (SU)} & \textbf{487} \\
\quad\textsc{Superficial Var Changes} & 100 \\ 
\quad\textsc{Step Omission} & 81 \\
\quad\textsc{Irrelevant Info} & 159 \\
\quad\textsc{Miscellaneous} & 147 \\
\toprule
\textbf{Total Instances} & \textbf{2391} \\
\midrule
\end{tabular}
\caption{Statistics of perturbations across categories and types.}
\label{tab:perturbations_stats}
\end{table}

==> tables/table4_gradewise_vs_perturbations_modelwise.tex <==
\setlength{\tabcolsep}{5pt} % Adjust column spacing
\renewcommand{\arraystretch}{1.3} % Adjust row spacing
\begin{table}[!t]
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11} & \textbf{12}\\
\midrule

% \multicolumn{9}{c}{\textit{Error Detection}} \\
\gptfouro & \normalsize 0.73 & \normalsize 0.57 & \normalsize 0.85 & \normalsize 0.83 & \normalsize 0.73 & \normalsize 0.77\\
\pixtral & \normalsize 0.73 & \normalsize 0.57 & \normalsize 0.85 & \normalsize 0.83 & \normalsize 0.73 & \normalsize 0.77\\
\bottomrule
\end{tabular}
\caption{Performance of VLMs across different grades. ($\uparrow$) indicate better performance.}
\label{tab:eval_non_cascaded}
\end{table}


==> tables/table9_cascaded.tex <==
\setlength{\tabcolsep}{5pt} % Adjust column spacing
\renewcommand{\arraystretch}{1.1} % Adjust row spacing
\begin{table}
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{A0} & \textbf{A1} & \textbf{B0} & \textbf{B1} & \textbf{C0} & \textbf{C1} & \textbf{D0}& \textbf{D1} & \textbf{E0} & \textbf{E1} \\
\midrule
\gptfouro & 425 & 1104 & 2 & 8 & 1 & 0 & 0 & 380 & 0 & 317 \\
\bottomrule
\end{tabular}
\caption{Numbers in Cascaded setup.}
\label{tab:cascaded}
\end{table}

